GANFusion: Feed-Forward Text-to-3D with Diffusion in GAN Space

We train a feed-forward text-to-3D diffusion generator for human characters using only single-view 2D data for supervision. Existing 3D generative models cannot yet match the fidelity of image or video generative models. State-of-the-art 3D generators are either trained with explicit 3D supervision and are thus limited by the volume and diversity of existing 3D data. Meanwhile, generators that can be trained with only 2D data as supervision typically produce coarser results, cannot be text-conditioned, or must revert to test-time optimization. We observe that GAN- and diffusion-based generators have complementary qualities: GANs can be trained efficiently with 2D supervision to produce high-quality 3D objects but are hard to condition on text. In contrast, denoising diffusion models can be conditioned efficiently but tend to be hard to train with only 2D supervision. We introduce GANFusion, which starts by generating unconditional triplane features for 3D data using a GAN architecture trained with only single-view 2D data. We then generate random samples from the GAN, caption them, and train a text-conditioned diffusion model that directly learns to sample from the space of good triplane features that can be decoded into 3D objects.

==> sections/figure_pages.tex <==
% \begin{figure}[p]
%     \includegraphics[width=\textwidth]{images/qualitative_comparison_cropped.pdf}
%     \caption{\textbf{Qualitative comparison.} We provide visual results from our method as well as the baselines. We provide random generations from AG3D~\cite{dong2023ag3d} which is unconditional. While random samples are of high quality, it is not straightforward to extend AG3D to enable text conditioning even with the addition of CLIP based losses during training. RenderDiffusion~\cite{anciukevivcius2023renderdiffusion} can follow the text prompts but lacks in terms of quality. \methodname matches the quality of AG3D while enabling text conditioning. For AG3D and our results, we visualize the results with the 2D upsampler trained jointly with the 3D GAN generator in the first stage of our method.}
%     \label{fig:comparison}
% \end{figure}






\begin{figure}[t]
    \includegraphics[width=\textwidth]{images/conditional_ag3d.pdf}
    \caption{\textbf{Text-conditional AG3D.} We attempt to add text conditioning to AG3D~\cite{dong2023ag3d} by providing text embeddings as additional input both to the generator and the dicriminator. However, we find that the training is not stable and does not converge.}
    \label{fig:conditional_ag3d}
\end{figure}

